Dueling Convex Optimization with General Preferences

We address the problem of \emph{convex optimization with dueling feedback}, where the goal is to minimize a convex function given a weaker form of \emph{dueling} feedback. Each query consists of two points and the dueling feedback returns a (noisy) single-bit binary comparison of the function values of the two queried points. The translation of the function values to the single comparison bit is through a \emph{transfer function}. This problem has been addressed previously for some restricted classes of transfer functions, but here we consider a very general transfer function class which includes all functions that can be approximated by a finite polynomial with a minimal degree $p$. Our main contribution is an efficient algorithm with convergence rate of $\smash{\widetilde O}(\epsilon^{-4p})$ for a smooth convex objective function, and an optimal rate of $\smash{\widetilde O}(\epsilon^{-2p})$ when the objective is smooth and strongly convex.

==> analysis_smooth.tex <==
\subsection{Convergence Analysis of \pgd\,(\cref{alg:pgd}) for Smoothly Convex Functions}
\label{sec:analysis_smooth}

\begin{restatable}[Convergence Analysis for Smoothly Convex Functions]{thm}{thmpgd}
\label{thm:pgd}
Consider a dueling feedback optimization problem parameterized  by any general admissible transfer function $\rho$ with \pprox\, $\rhoo$ and a $\beta$ smooth convex function $f: \cD \mapsto \R$. 
%Also let in Alg. \ref{algo:grad} the initial point $\w_1$ is such that $f(\w_1) - f(\w^*) > \epsilon$. 
Then given any $\epsilon > 0$, for the choice of $\gamma = \frac{\tc \epsilon}{\beta \sqrt{d}\holdon}$ and $\eta = \frac{pc_\rho \tc^{2p-1} \epsilon^{2p}}{d^{(2p+1)/2}\beta^p \holdon^{2p-1}}$, there exists at least one $t$ such that $\E[f(\w_{t})] - f(\w^*) \le \epsilon$, after at most $T = \frac{d^{2p+1}\beta^{2p} \holdon^{4p}}{p^2 (\tc^{p2-1} c_\rho)^2\epsilon^{4p}}+1$ iterations;  i.e. $\min_{t \in [T]}\E[f(\w_{t})] - f(\w^*) \le \epsilon$, where $\tc \in [\tfrac{1}{20},1]$ is a universal constant as indicated in \cref{lem:normgrad}.
\end{restatable}

\begin{rem}[Universality of \kgd\, for any general transfer functions.]
\label{rem:pgd_interpolate}
\cref{thm:pgd} shows that for any general transfer function $\rho$ with a $p$-th degree \pprox\, $\rhoo$, \cref{alg:pgd} gives a convergence rate of $O(\epsilon^{-4p})$ to find an $\epsilon$-optimal point. However, \cref{thm:pgdi} shows a improved convergence rate of $O(\epsilon^{-3})$ for linear $(p=1)$ transfer functions which recovers the convergence rate obtained in \cite{sahatewari} for smooth convex functions in the \emph{Bandit Convex Optimization} ($1$ point feedback setting). Moreover, \cref{thm:pgd} also shows how \cref{alg:pgd} can yield a faster convergence rate of $O(\epsilon^{-1})$ for $\sign$ transfer functions $(p=0)$ which matches the convergence rate obtained in \cite{SKM21} --- in fact, not just the final convergence rate, our algorithm (\kgd, \cref{alg:pgd}) generalizes the $\beta$-NGD algorithm of \cite{SKM21} since our descent direction estimate $(\g_t)$, exactly behaves like the normalized gradient (gradient direction) at point $\w_t$ which was the crux of their optimization analysis. Please see the proof of \cref{thm:pgdi} for more details.
\end{rem}

\begin{proof}[\textbf{Proof Sketch of \cref{thm:pgd}}]
The complete details of the proofs can be found in \cref{app:pgd}. 
%
We denote by $\cH_t$ the history $\{\w_\tau,\u_\tau,o_\tau\}_{\tau = 1}^{t-1} \cup \w_{t}$ till time $t$.
%
We start by noting that by definition: 
\[
\E_{o_t}[\g_t \mid \cH_t,\u_t] = \rho(f(\w_t+\gamma \u_t) - f(\w_t - \gamma \u_t))\u_t
\]

\textbf{Base Case:} Let us start with the assumption that $f(\w_1)-f(\w^*) > \epsilon$ (as otherwise we already have $\min_{t \in [T]}\E[f(\w_{t})] - f(\w^*) \le \epsilon$ and there is nothing to prove).

We proceed with the proof inductively, i.e. given $\cH_t$ and assuming (conditioning on) $f(\w_t) - f(\w^*) > \epsilon$, we can show that $\w_{t+1}$ always come closer to the minimum $\w^*$ on expectation in terms of the $\ell_2$-norm. More formally, given $\cH_t$ and assuming  $f(\w_t) - f(\w^*) > \epsilon$ we will show:
%
$
\E_t[\norm{\w_{t+1}-\w^*}^2] \leq \norm{\w_{t}-\w^*}^2,
$ %but this might not imply f(\w_{t+1})-f(\w^*) < const  f(\w_{t})-f(\w^*)  which is true in the strongly convex case though...
%
where $\E_t[\cdot]:= \E_{o_t,\u_t}[\cdot \mid \cH_t]$ denote the expectation with respect to $\u_t,o_t$ given $\cH_t$. The precise statement can be summarized in the following lemma:

\begin{restatable}[Roundwise Progress of \kgd]{lem}{lempgd}
\label{lem:pgd}
Consider the problem setup of \cref{thm:pgd} and also the choice of $\eta$, $\gamma$. 
%
Then at any time $t$, during the run of \kgd~(\cref{alg:pgd}), given $\cH_t$, if $f(\w_t) - f(\w^*) > \epsilon$, we can show that:
\begin{align}
\label{eq:fin1orig}
    \E_t[\norm{\w_{t+1}-\w^*}^2] \leq \norm{\w_{t}-\w^*}^2 - \frac{p^2 (\tc^{2p-1} c_\rho)^2\epsilon^{4p}}{d^{2p+1}\beta^{2p} \holdon^{4p-2}}
\end{align}
\end{restatable}

\begin{proof}
We first note that by our update rule,

\begin{align}
\label{eq:ub1orig}
    \E_t[\norm{\w_{t+1}-\w^*}^2] 
    &\leq 
    \E_t[\norm{\w_{t}-\w^*}^2] - 2\eta \E_t[\brk[s]{ \g_t \dotp (\w_t-\w^*) }] + \eta^2 \nonumber
    \\
    &=
    \norm{\w_{t}-\w^*}^2 - 2\eta \E_t[\brk[s]{ \g_t \dotp (\w_t-\w^*) }] + \eta^2 
    .
\end{align}
% 

\textbf{Assumptions: } Let us assume

On the other hand,
\begin{align}
	\label{eq:lb1}
    & \E_t [\g_t \dotp (\w_t-\w^*)] 
    = 
    \E_{\u_t} \brk[s]!{ \rho\brk{ f(\w_t + \gamma \u_t) - f(\w_t - \gamma \u_t) } \u_t \dotp (\w_t-\w^*) \mid \cH_t } \nonumber
    \\
    &= 
    \E_{\u_t} \brk[s]!{ \abs!{\rho\brk{ f(\w_t + \gamma \u_t) - f(\w_t - \gamma \u_t) }} \cdot \abs!{\u_t \dotp (\w_t-\w^*)} \mid \cH_t } \nonumber
    \\
    &\geq
    \E_{\u_t} \brk[s]!{ \abs!{\rhoo\brk{ f(\w_t + \gamma \u_t) - f(\w_t - \gamma \u_t) }} \cdot \abs!{\u_t \dotp (\w_t-\w^*)} \mid \cH_t } \nonumber
    \\
    &=
    \E_{\u_t} \brk[s]!{ \rhoo\brk{ f(\w_t + \gamma \u_t) - f(\w_t - \gamma \u_t) } \cdot \u_t \dotp (\w_t-\w^*) \mid \cH_t } \nonumber
    \\
    &= 
    \frac{\gamma}{d}\E_{\u_t}\brk[s]!{ \rhoo'\big( \abs{f(\w_t+\gamma\u_t) - f(\w_t-\gamma\u_t)} \big) \big( \nabla f(\w_t+\gamma\u_t) + \nabla f(\w_t-\gamma\u_t) \big) \mid \cH_t } \dotp (\w_t-\w^*) 
    ,
\end{align}
where the inequality follows by the definition of $\rhoo$ which is \pprox\, of $\rho$ (see \cref{def:rhoo}).   
% 
Now, using convexity of $f$ and $\beta$-smoothness, we can further show that:

\begin{align}
\label{eq:may20}
&	\E_{t} [\g_t \dotp (\w_t-\w^*)] 
    \geq
    \frac{2\gamma}{d} \E_{\u_t}\brk[s]!{ \rhoo'\big( \abs{ f(\w_t+\gamma\u_t) - f(\w_t-\gamma\u_t) } \big) \brk!{ f(\w_t) - f(\w^*) - \beta \gamma^2 } },
	\\
&  \text{and also } \E_{\u_t}[\abs*{ f(\w_t+ \gamma \u_t) - f(\w_t-  \gamma \u_t)}] \geq \E_{\u_t}[\abs{2 \gamma \u_t \dotp \nabla f(\w_t) }] - \beta \gamma^2
= 2\frac{\tc \gamma \norm{\nabla f(\w_t)} }{\sqrt{d}} - \beta \gamma^2 \nonumber
\end{align}
where the last equality is due to \cref{lem:normgrad}.
%
Additionally, since we assumed $f(\w_t)-f(\w^*) > \epsilon$, i.e. the suboptimality gap to be at least $\epsilon$, by \cref{lem:gradf_lb} we can further derive a lower bound: 
\begin{align*}
\E_{\u_t}[\abs*{ f(\w_t+ \gamma \u_t) - f(\w_t-  \gamma \u_t)}] \geq \frac{2\tc \gamma \epsilon}{\sqrt{d}\norm{\w_t - \w^*}} - \beta \gamma^2 
= {\frac{2\tc \gamma \epsilon}{\sqrt{d}D}} - \beta \gamma^2. 
\end{align*}
%
Now for the choice of $\gamma = \frac{\tc \epsilon}{\beta \sqrt{d}\holdon}$ since the lower bound in right hand side is always positive, by monotonicity of $\rhoo'$ in the +ve orthant we get: 

 \begin{align}
 \label{eq:may21}
 \rhoo'(\E_{\u_t}[\abs*{ f(\w_t+ \gamma \u_t) - f(\w_t -  \gamma \u_t)}]) \geq \rhoo'\bigg( {\frac{\tc^2 \epsilon^2}{\beta {d}D^2}} \bigg) = c_\rho p \bigg( {\frac{\tc^2 \epsilon^2}{\beta {d}D^2}} \bigg)^{p-1},
 \end{align}
where the last equality follows since by definition $\rho'(x) = c_\rho p x^{p-1} \text{ for any } x \in \R_+$.  
Finally combining \cref{eq:may20,eq:may21}, and the choice of $\gamma$, we can finally derive the lower bound: 
\vspace{-1pt}
\begin{align}
	\label{eq:lb4orig}
	\E_{t} [\g_t \dotp (\w_t-\w^*)] 
	\geq 
	\frac{pc_\rho \tc^{2p-1} \epsilon^{2p}}{d^{(2p+1)/2}\beta^p \holdon^{2p-1}}
	,
\end{align}
\vspace{-5pt}
Combining \cref{eq:ub1orig} with \cref{eq:lb4orig}:
\vspace{-5pt}
\begin{align}
    \E_t & [\norm{\w_{t+1}-\w^*}^2] 
    \leq 
    \norm{\w_{t}-\w^*}^2 - 2\eta \E_t[\brk[s]{ \g_t \dotp (\w_t-\w^*) }] + \eta^2 \nonumber
   \leq \nonumber 
    \norm{\w_{t}-\w^*}^2
     - 2\eta \Bigg( \frac{pc_\rho \tc^{2p-1} \epsilon^{2p}}{d^{(2p+1)/2}\beta^p \holdon^{2p-1}} \Bigg) + \eta^2
     \\
    & \leq  
    \norm{\w_{t}-\w^*}^2
    - \Bigg( \frac{pc_\rho \tc^{2p-1} \epsilon^{2p}}{d^{(2p+1)/2}\beta^p \holdon^{2p-1}} \Bigg)^2, ~~\text{ setting } \eta = \Bigg( \frac{pc_\rho \tc^{2p-1} \epsilon^{2p}}{d^{(2p+1)/2}\beta^p \holdon^{2p-1}} \Bigg) \nonumber 
    ,
\end{align}
which concludes the claim of \cref{lem:pgd}.
\end{proof}

Now coming back to the main proof of \cref{thm:pgd}, note by iteratively taking expectation over $\cH_T$ on both sides of \cref{eq:fin1orig} and summing over $t=1,\ldots,T$, we get,

\begin{align*}
	\E_{\cH_T} [\norm{\w_{T+1}-\w^*}^2] 
	& \leq 
	\norm{\w_{1}-\w^*}^2
	- \frac{p^2 (\tc^{2p-1} c_\rho)^2\epsilon^{4p}}{d^{2p+1}\beta^{2p} \holdon^{4p-2}}T	 
	.
\end{align*}
%\vspace{-5pt}
However, note if we set $T = \frac{d^{2p+1}\beta^{2p} \holdon^{4p}}{p^2 (\tc^{2p-1} c_\rho)^2\epsilon^{4p}}$,
this implies 
$\E_{\cH_T} [\norm{\w_{T+1}-\w^*}^2] \leq 0$, or equivalently $\w_{T+1} = \w^*$, which concludes the claim. 

To clarify further, note we show that for any run of Alg. \ref{alg:pgd} if indeed $f(\w_{t}) - f(\w^*) > \epsilon$ continues to hold for all $t = 1,2, \ldots T$, then $\w_{T+1} = \w^*$ at $T = \frac{d^{2p+1}\beta^{2p} \holdon^{4p}}{p^2 (\tc^{2p-1} c_\rho)^2\epsilon^{4p}}$. If not, there must have been a time $t \in [T]$ such that $f(\w_t) - f(\w^*) < \epsilon$. %This concludes the proof with $T_\epsilon = T$.
\end{proof}	

	








